Towards Designing a Self-Managed Machine Learning Inference Serving System inPublic Cloud

We are witnessing an increasing trend towardsusing Machine Learning (ML) based prediction systems, span-ning across different application domains, including productrecommendation systems, personal assistant devices, facialrecognition, etc. These applications typically have diverserequirements in terms of accuracy and response latency, thathave a direct impact on the cost of deploying them in a publiccloud. Furthermore, the deployment cost also depends on thetype of resources being procured, which by themselves areheterogeneous in terms of provisioning latencies and billingcomplexity. Thus, it is strenuous for an inference servingsystem to choose from this confounding array of resourcetypes and model types to provide low-latency and cost-effectiveinferences. In this work we quantitatively characterize the cost,accuracy and latency implications of hosting ML inferenceson different public cloud resource offerings. In addition, wecomprehensively evaluate prior work which tries to achievecost-effective prediction-serving. Our evaluation shows that,prior work does not solve the problem from both dimensionsof model and resource heterogeneity. Hence, we argue that toaddress this problem, we need to holistically solve the issuesthat arise when trying to combine both model and resourceheterogeneity towards optimizing for application constraints.Towards this, we envision developing a self-managed inferenceserving system, which can optimize the application require-ments based on public cloud resource characteristics. In orderto solve this complex optimization problem, we explore the highlevel design of a reinforcement-learning based system that canefficiently adapt to the changing needs of the system at scale.

==> backups/bkp_1-introduction.tex <==
Sustained advances in Machine Learning (ML) has fueled \st{the extensive use of prediction from ML models by various} many applications such as product recommendation systems~\cite{shaya2010intelligent}, facial recognition~\cite{bartlett2005recognizing}, intelligent personal assistants~\cite{sirius}, etc. \st{Especially,} Among many ML paradigms, Artificial Deep Neural Networks (DNNs), thanks to their generalization and massively parallel nature, has been predominant in making all these applications pervasive and accessible to common men. \st{constitute a major part of these prediction models}. A typical DNN model has two different phases, namely, \textit{training} and \textit{inference}. Training a DNN, which is the process of extracting and learning the patterns and the features from millions of sample-data,  typically takes a few hours to days (depending on the complexity, depth and number of parameters in the model). The trained models are hosted as web-service, which are often queried for predictions during the inference phase. There has been enormous attention given towards training these ML models for better accuracy and convergence time. However, prediction serving is also equally challenging. 
\begin{figure}[ht!]
\centering
\begin{minipage}{0.99\linewidth}
\begin{center}
\includegraphics[width=0.9\textwidth]{figures/multi-staged.pdf}
%\end{minipage}
\caption{Typical architecture of hosting a prediction-based system hosted in public cloud.}
\label{fig:architecture}
\end{center}
\end{minipage}
\end{figure}
These prediction queries are typically administered with strict response latencies, which are usually under 1s. Apart from latency, throughput is also an essential consideration for companies like Facebook~\cite{facebook}, which serve tens to trillions of inference queries every day. The latency and throughput of these queries are governed by multiple factors~\cite{8327042}.

%Models that require high accuracy are known to have longer running times compared to models that require low accuracy. 
Based on the nature of the application, each of them has different accuracy, latency, and cost requirements. For example, a facial tag recommendation in social networks, product recommendation systems, etc, will have strict response latencies but can tolerate lower accuracy. On the other hand, for personal assistant systems like speech translation, having higher accuracy is critical. To ensure a required accuracy, applications can choose from different types of NN models, which by themselves have diverse response latencies. Therefore it is \emph{non-trivial for an application to choose the right model which can optimize for all requirements together}.  

Unlike accuracy and latency which can be controlled by choosing the right model, the cost depends on the type of deployment used to host these models in a public cloud. The deployment costs differ based on the provisioning times and longevity of the resource procured. Typically these inference serving systems are hosted using Virtual Machines, which takes a few minutes to start-up. Due to high start-up latencies~\cite{vm_startup}, using VMs for hosting ML services can lead to over-provisioning, especially during periods of poor workload predictability (flash crowds)~\cite{Urgaonkar:2008:ADP:1342171.1342172,Urgaonkar:2002:ROA:844128.844151}. In stark contrast to VMs, serverless functions have been made available by cloud providers, which can spin-up within a few seconds~\cite{firecracker}. As we will discuss in this paper, the cost of using VMs vs serverless functions highly depends on the dynamically varying needs of the end-user query submission rates. 

Besides workload arrival rates, there is further variability in terms of configuring serverless functions to meet the end user demands of latency and cost requirements. This is because, these functions are billed as a function of number of invocations, compute time and memory requirement by the function. As we note in this paper, \emph{the memory allocated per function is inversely proportional to compute time and directly proportional to billing cost}. 

Therefore, these clear deficiencies in terms of choosing the right resource type and selecting the appropriate model type for a given user requirement motivates the central question of this work: \emph{does there exist an optimal resource procurement system which can balance the goals of diverse user requirements for accuracy, latency and cost by efficiently mapping model parameters to heterogeneous resource specifications?} Our preliminary results suggest that using a combination of VMs and Serverless functions could potentially solve this optimization problem. As opposed to prior work~\cite{mark,infaas,spock}, which try to combine serverless functions with VMs to hide the start-up latencies of VMs, in this work we explore different \textbf{key aspects} with respect to blending serverless function with VMs to host NN-based ML prediction serving systems in public cloud as given below.

$\bullet$ \textbf{Model Selection:} How to make the users oblivious to resource selection and model selection which map to their cost, accuracy, and latency requirements?

$\bullet$ \textbf{Heterogeneous Resources:} What are the different options available in terms of combining different VM-based cloud services and serverless functions for a given user requirement?

$\bullet$ \textbf{Configuring Resources:} From the diverse options, how to right size VMs and configure the serverless function appropriately to efficiently cater to user specified cost, accuracy and latency constraint? 

$\bullet$ \textbf{Bring in Tune}: Based on dynamically changing query arrivals over time, what is the right degree to mix and match serverless functions along with VMs without compromising the user specified requirements?

By exploring these key aspects, we envision to develop a self-managed ML-prediction system, which can cater to different diverse needs of applications by leveraging the diverse resource availability from public cloud. We emphasize that, prior work~\cite{infaas} in this field, still suffer from over-provisioned virtual machines in case of dynamic arrivals to satisfy response latency. To address this challenge, we explore the option to use serverless function along with VMs and discuss the challenges in deploying such a mixed resource procurement system. Further, we propose to develop a reinforcement learning-based system, which can dynamically adapt to the changing application needs and public cloud offerings. \vspace{-2mm}%explore the possibility of using mixed resource procurement for applications apart from prediction-based systems. 



% Importance of machine learning used for inference and product recommendation services etc. 

% How response latency is critical for these services.

% How diverse these ML models are in terms of parameters like accuracy, performance and how they affect the latency. Implications of these parameters for a given user constraint in terms of cost and SLO. 

% Typically how they are hosted in public cloud using Virtual Machines. How cost is dependent on resource provisioning and latency. What are the drawbacks of using VMs and how Serverless functions help alleviate them.
% Configuring serverless functions and VMs catering to the latency and accuracy constraints has implications on cost. 

% Still matching the constraints of the user by combining all the model parameters and procuring the right resources is a challenge. How can we mix and match VMs and lambdas to offer better SLO under give cost constraint. 




